GreenFPGA: Evaluating FPGAs as Environmentally Sustainable Computing Solutions

Growing global concerns about climate change highlight the need for environmentally sustainable computing. The ecological impact of computing, including operational and embodied, is a key consideration. Field Programmable Gate Arrays (FPGAs) stand out as promising sustainable computing platforms due to their reconfigurability across various applications. This paper introduces GreenFPGA, a tool estimating the total carbon footprint (CFP) of FPGAs over their lifespan, considering design, manufacturing, reconfigurability (reuse), operation, disposal, and recycling. Using GreenFPGA, the paper evaluates scenarios where the ecological benefits of FPGA reconfigurability outweigh operational and embodied carbon costs, positioning FPGAs as a environmentally sustainable choice for hardware acceleration compared to Application-Specific Integrated Circuits (ASICs). Experimental results show that FPGAs have lower CFP than ASICs, particularly for multiple distinct, low-volume applications, or short application lifespans.

==> misc/customize.tex <==
\usepackage{float} 
\usepackage{tabularx}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{hhline}
\usepackage{silence}
\usepackage{graphicx}
\usepackage{multirow} 
\usepackage{graphicx}
\usepackage{multirow}
\usepackage[english]{babel}
\usepackage{booktabs}
\usepackage{array}
\usepackage{paralist}
\usepackage{threeparttable}
\usepackage{lipsum}
\usepackage{flushend}
\usepackage{cuted}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{algcompatible}
\usepackage{color}
\usepackage{psfrag}
\usepackage{epsfig}
\usepackage{multicol}
\usepackage{color}
\usepackage{fancybox}
\usepackage{subfigure}
\usepackage{cite}
\usepackage{theorem}
\usepackage{url}
\usepackage[table]{xcolor}
\usepackage{epstopdf}
\usepackage[normalem]{ulem}
\usepackage{siunitx}
\usepackage{rotating}

%\usepackage{biblatex} 
%\usepackage[backend=biber]{biblatex}
%\usepackage[style=apa,sortcites=true,sorting=nyt,backend=biber]{biblatex}
%\usepackage{subcaption}
\usepackage[justification=centering,font=small,labelfont=bf]{caption}
% \usepackage[font=small,labelfont=bf]{caption}
\usepackage{silence}
\WarningFilter{caption}{Unsupported document class}
\usepackage{enumitem}
%\usepackage{widetext}
%\usepackage{paralist}
%\usepackage[none]{hyphenat}
\hyphenation{intersection op-tical net-works semi-conductor Electro-migration immortality}
\definecolor{gray1}{gray}{0.90}
\definecolor{gray2}{gray}{0.98}
\definecolor{light-gray}{gray}{0.95}
\def\bibfont{\scriptsize}
%Adds extra padding to the table cells
\setlength\extrarowheight{2pt}

\newcommand{\ignore}[1]{}
\newcommand{\redHL}[1]{\textcolor{red}{#1}}
\newcommand{\redfn}[1]{\textcolor{red}{\footnote{\textcolor{red}{#1}}}}
\newcommand{\blueHL}[1]{{\textcolor{blue}{#1}}}
\newcommand{\greenHL}[1]{\textcolor{green}{#1}}
\newcommand{\blackHL}[1]{\textcolor{black}{#1}}
\newcommand{\Alter}[2]{\sout{#1}\redHL{#2}}
\newcommand{\txtoverline}[1]{$\overline{\mbox{{#1}}}$}
\newcommand{\TMR}{\mbox{TMR}}
\newcommand{\sTMR}{\scriptsize{\mbox{TMR}}}
%\newcommand{\Deff}{D_{\mbox{\tiny \em eff}}}
%\newcommand{\Deffn}{D_{\mbox{\tiny \em eff,n}}}
%\newcommand{\Deffg}{D_{\mbox{\tiny \em eff,g}}}
%\newcommand{\Zeff}{Z^\star_{\mbox{\tiny \em eff}}}
%\newcommand{\Javg}{J_{\mbox{\tiny \em avg}}}
%\newcommand{\Jeff}{J_{\mbox{\tiny \em eff}}}
%\newcommand{\Jrms}{J_{\mbox{\tiny \em rms}}}
%\newcommand{\Jflux}{J_{\mbox{\tiny \em flux}}}
%\newcommand{\vivekeq}[1]{\mbox{\tiny {\em #1}}}
%\newcommand{\Tlife}{T_{\mbox{\tiny \em life}}}
%\newcommand{\Ieff}{I_{\mbox{\tiny \em eff}}}
%\newcommand{\Irise}{I_{\mbox{\tiny \em rise}}}
%\newcommand{\Jpavg}{J_{\vivekeq{avg}}^+}
%\newcommand{\Jnavg}{J_{\vivekeq{avg}}^-}
%\newcommand{\Jbavg}{J_{\vivekeq{avg}}^{\vivekeq{blue}}}
%\newcommand{\Jgavg}{J_{\vivekeq{avg}}^{\vivekeq{green}}}
%\newcommand{\nuc}{t_{\mbox{\scriptsize \it nuc}}}
%\newcommand{\nucs}{t_{\mbox{\scriptsize \it nuc--SI}}}
%\newcommand{\nucf}{t_{\mbox{\scriptsize \it nuc--F}}}
%\newcommand{\tlife}{t_{\mbox{\scriptsize \it life}}}
%\newcommand{\Mx}{\mbox{M}_{\mbox{\scriptsize x}}}
%\newcommand{\Mxp}{\mbox{M}_{\mbox{\scriptsize x+1}}}
\pagestyle{plain}
\renewcommand{\bibfont}{\tiny}
\usepackage{tikz}
\usetikzlibrary{tikzmark}
%\usetikzlibrary{shapes,arrows}
\renewcommand{\baselinestretch}{0.93}
%\selectcolormodel{gray}


==> sec/old_outline/4-heterogeneous-fpga.tex <==
\section{Heterogeneous FPGA/Optimum FPGA workload allocation}
\label{sec:results}

\subsection{FPGA Workload balancing}
Workload distribution between FPGA, CPU, GPU, and AI-Accelerators for best and optimum performance and lowest CFP
Look for test cases in AI/ML ; Autonomous ; etc

\subsection{CFP based FPGA design}
Designing FPGA based on CFP of FPGA building blocks
\begin{enumerate}
    \item LUT
    \item DSP
    \item Memories
    \item ALM
    \item etc 
\end{enumerate}

\noindent
%{\it (1) Input parameters} Our CFP estimator, developed in Python3.7,  uses several input parameters which are listed in Table I with their supported range of values and their sources. For instance, based on the source of energy, whether it is coal, gas, wind etc, the $C_\text{mfg, src}$ can be a value between 30g -- 700g of CO$_2$ or based on the technology node, the defect densities can be between 0.07 -- 0.3/cm$^2$~\cite{lau22}. 

%Although our simulator can handle a range of technology nodes for packaging and a range of derate factors for $C_\text{mfg, src}$, as highlighted in the table, our results in this section are shown for specific values, i.e., we assume all packaging technology (RDL, EMIB, and active/passive interposers) to be in 65nm and the energy source is from coal at 700g of CO$_2$ per KWh. Based on the testcase, we vary the technology node for each of the chiplets to explore the possible design space and estimate $C_\text{mfg}, i$. Based on the technology each chiplet is implemented in,  we choose the appropriate values from the specified ranges.


\begin{comment}
\begin{table}[tb]
\centering
\label{tbl:knobs}
\caption{List of input parameters to our embodied CFP estimation tool and their range of values and sources.}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{c|crll}
\hline
Model   &     Parameter     &     Value&Unit     &     Source   \\ \hline
 \multirow{8}{*}{$C_{\text{mfg},i}$ }     & $D0(p)$           &  0.07 -- 0.3&/cm$^2$  & \cite{supply-chain, active-vs-passive-2} 
\\ %\hline
    &     $\alpha$         &   3&     &    \cite{supply-chain, active-vs-passive-2}    
 \\ %\hline
      &      $D_T(d, p)$     &  5 -- 150&MTr/mm$^2$    &\cite{tsmc-transistor-density, tsmc-sram-scaling} 
 \\ %\hline
     &      $\eta_{eq}(p)$  &  0 -- 1&   &  \cite{TSMC-report}  
 \\ %\hline
    &      $C_\text{mfg, src}$ & 30 -- 700&g CO$_2$/kWh   & \cite{act, imec-dtco}  
 \\ %\hline
    &    $\text{EPA}(p)$        &   0.8 -- 3.5 &kWh/cm$^2$       &    \cite{act, imec-dtco}         
  \\ %\hline

    &    $C_\text{gas}$        &   0.1 -- 0.5&kg CO$_2$/cm$^2$       &    \cite{act, imec-dtco}            
  \\% \hline

     &    $C_\text{material}$        &   0.5& kg CO$_2$/cm$^2$        &    \cite{act, imec-dtco}             
  \\ \hline
  
 \multirow{8}{*}{$C_\text{package}$}      &     RDL tech.      &     22nm - 65nm&   &  \cite{lau22, emib, active-passive-interposers}  
 \\ %\hline
&    $\text{EPLA}_\text{RDL}(p)$        &      0.05 -- 0.2 &kWh/cm$^2$   &    \cite{act, imec-dtco}         
\\% \hline
      &      $C_\text{pkg, src}$ & 30 -- 700&g CO$_2$/kWh   &  \cite{act, imec-dtco} 
 \\% \hline
    &      $L_{RDL}$ & 3 -- 4& & \cite{lau22} 
 \\% \hline
   &     $L_\text{bridge}$ & 3 -- 4& & \cite{emib} 
 \\% \hline
    &     Bridge tech.      &     22nm -- 65nm&    &  \cite{emib}  
 \\% \hline
      &    $\text{EPLA}_\text{bridge}(p)$        &   0.1 -- 0.35& kWh/cm$^2$     &    \cite{act, imec-dtco}          
 \\% \hline
      &    Bridge range & 2 $\times$ 2&mm$^2$ & \cite{emib} 
 \\ \hline
 \multirow{2}{*}{$C_\text{mfg,comm}$}      &     Interposer tech.      &     22nm -- 65nm&    & \cite{active-passive-interposers}   
 \\% \hline

   &     NoC flit width.      &     512 bits&    & \cite{active-passive-interposers}   
 \\ \hline

$C_\text{whitespace}$      &     Chiplet spacing      &     0.1 -- 1 & mm   &  \cite{active-passive-interposers, chiplet_spacing}  
 \\ \hline

\multirow{4}{*}{$C_\text{des}$}    &  $\eta_\text{EDA}$     &     0 -- 1&   &  \cite{eda-tool-scaling}   
 \\% \hline

 &  $P_\text{des}$     &   10&W     & \cite{power-per-core}   
 \\% \hline

  &  $N_\text{des}$     &     100&   & \cite{abk-schedule}   
 \\ % \hline
 & $C_\text{des, src}$ & 30 -- 700 & g CO$_2$/kWh   &  \cite{act, imec-dtco}  
  \\ \hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}
\end{comment}


\noindent
%{\it (2) Testcases and architectures}
%We evaluate our carbon simulator on four industry testcases: (i) Intel mobile processor, Tiger Lake(2020)~\cite{tigerlake-die-area}, (ii) Intel server-class 2-chiplet-based  CPU, Emerald Rapids (EMR)~\cite{emr-die-area} (to be released in Q4 2023), (iii) NVIDIA GA102 GPU (2020)~\cite{ga102-die-area}, and (iv) Apple A15 SoC (2021)~\cite{a15-wiki}. The input to our simulator is an architectural description of these testcases with the die area breakdowns for each of these processors. We obtain the area breakdowns of each of these testcases from third-party websites such as~\cite{emr-die-area, ga102-die-area, a15-die-area, tigerlake-die-area}. For the monolithic SoCs (Tiger Lake, GA102, and A15) we break them into chiplets based on the block-level architecture. We use one chiplet for memory, another chiplet for analog components, and a third chiplet for digital logic inspired by~\cite{AMD-Zen2}. We also further explore the design space by splitting the large digital logic chiplet into smaller chiplets. For Intel Emerald Rapids, an EMIB-based 2-chiplet testcase, we perform CFP estimation for the original chiplet-based architecture. We also perform carbon evaluation on a 4-chiplet version of the same testcase where we split the large digital logic blocks into two smaller chiplets each.  

%In the rest of this section, we use the NVIDIA GA102 testcase as a case study and show detailed results on each of the components (manufacturing, packaging, and design) of the total embodied CFP for different possible chiplet architectures and compare it to the CFP of the monolithic SoC. 
%Next, in the interest of space, for the rest of the three testcases, we only summarize the manufacturing and packaging CFP and compare that to its monolithic counterpart. 


==> sec/old_outline/5-results.tex <==
\section{Results}
\label{sec:results}

For this, we need sweep the following values:
Embodied CFP to Operational CFP of the ASIC for just 1 application
Embodied CFP is increasing as we go into the future
When E:O is higher, then FPGAs are becoming sustainable
Power efficiency ratio between ASIC and FPGA
Area efficiency ratio between ASIC and FPGA
Lifetime of the application
If it’s small, then FPGAs are more sustainable


%\subsection{Example case study: NVIDIA GPU GA102}
%As an example case study, we use the NVIDIA GPU GA102 architecture to evaluate the various components of embodied CFP for various chiplet disaggregation scenarios of the testcase.  The first set of results is for three-chiplet scenario where one of the chiplets implements memory, the other analog components, and the third digital blocks. The next set of results will show the CFP for a general $N_c$-chiplet architecture. 

\noindent
%\textit{(1)} \underline{\it Manufacturing and packaging CFP for three chiplets} The manufacturing CFP of GA102, for different configurations of technology nodes for each chiplet, is shown in Fig.~\ref{fig:cfp}(a). The x-axis lists the technology nodes where the lowermost row is the technology node for the digital logic, the middle row is analog components (IOs), and the topmost row is memory. The (7,7,7) scenario is a monolithic representation of the architecture of a single die in a 7nm node. It, therefore, does not have the additional HI-related packaging overheads, but includes packaging overheads as a part of manufacturing carbon using models from~\cite{act}. The figure shows that the lowest embodied CFP is for the (7, 14, 10) scenario. This is because the analog components and memory blocks~\cite{AMD-Zen2} do not scale in the area as much as the digital blocks and can therefore be implemented in an older technology node with almost the same area.  On the contrary, in the (10, 10, 10) scenario, the digital logic scales to a much larger area and therefore has a larger CFP than even the monolith resulting in a larger CFP even though the 10nm node has a lower defect density and lower CFPA when compared to 7nm. The packaging overhead values in this figure are for an RDL-based package with the RDL layers implemented in a 65nm technology node.  The packaging overhead has also accounted for the whitespace between the three chiplets and routing overheads. From this result, it is clear that HI enables using chiplets that have small areas and higher yields, which helps lowers the CFP, and the further integration of chiplets in different technology nodes can further lower the CFP as older nodes have lower $\text{EPA}$ than advanced nodes. 


\begin{comment}
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figs/cfp.png}
\vspace{-4mm}
\caption{(a) Manufacturing and packaging CFP, (b) design CFP for a {\bf single iteration} of SP\&R, and (c) overall CFP for different configurations of three chiplets for the NVIDIA GA102 architecture with RDL fan-out package. }
\vspace{-7mm}
\label{fig:cfp}
\end{figure}
\end{comment}




\noindent
%\textit{(2)} \underline{\it Design CFP for three chiplets}
%From our experiments in performing SP\&R of large designs, we find that the $t_{\text{SP\&R}, i}$ for a design with 700,000 logic gates in a 7nm commercial technology is about 24 CPU hours. These estimates are on a 192GB RAM machine with a dual-core Intel Xeon CPU with 8 threads, each running at a 2.4GHz clock frequency.  Therefore, extending this model to the NVIDIA GA102 testcase, $t_{\text{SP\&R},i} = 1.2\times 10^6$ CPU hours as it has over 4.5B logic gates. Assuming $P_\text{des} = 10$W~\cite{power-per-core} and the energy supplied comes from non-renewable sources, then a single run of SP\&R results in 8,400kg of CO$_2$ equivalent emission in the 7nm technology node. Fig.~\ref{fig:cfp}(b), shows the design carbon for a {\bf single iteration} of SP\&R for the three chiplet testcase. Older technology nodes have lower design times due to EDA tool scaling~\cite{eda-tool-scaling}, and therefore, have lower CFP when compared to the monolithic SoC in an advanced 7nm technology. 
%In addition, since HI enables the ``reuse" of pre-designed chiplets, in principle, the entire digital logic chiplet can be reused for another design saving the entire associated design CFP.


%Although, the CFP values in Fig.~\ref{fig:cfp}(b) are significantly large, these costs are amortized across the number of parts manufactured ($N_p$). The figure only shows the results for a single iteration of SP\&R. However, with hundreds ($N_\text{des} = 100$) of design iterations and SP\&R runs and verification dominating 80\% of the product development time, the design of an IC can easily contribute to over 2,000,000kg of CO$_2$ equivalent emission, assuming all compute energy is coming from non-renewable sources. Assuming the number of manufactured parts is $N_P=200,000$, the SP\&R carbon cost gets amortized to 12kg of CO$_2$ equivalent emission per IC, which is more than 25\% of the manufacturing carbon cost (see Fig.~\ref{fig:cfp}(a)).


\noindent
%\textit{(3)} \underline{\it Total embodied CFP for three-chiplet architecture}
%To estimate the total embodied CFP, we sum the manufacturing and packaging costs from Fig.~\ref{fig:cfp}(a) and amortized design costs assuming, $N_p = 200,000$ and $N_\text{des} = 100$ from Fig.~\ref{fig:cfp}(b).  Fig.~\ref{fig:cfp}(c) shows the total embodied CFP of all three components for different configurations of the three chiplet-based GA102 testcase.  The (7, 14, 10) configuration has the least CFP showing the potential of HI to bringing down CFP. 

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=0.75\linewidth]{figs/cfp-nc-chiplets.png}
\vspace{-3mm}
\caption{$C_\text{mfg}$ and $C_\text{HI}$ for $N_c$ chiplets on the NVIDIA GA102 GPU testcase.}
\vspace{-5mm}
\label{fig:cfp-nc-chiplets}
\end{figure}
\end{comment}

\noindent
%\textit{(4)} \underline{\it Total embodied CFP with $N_c$ chiplets} In addition to the three chiplet architecture of GA102, we also evaluate the manufacturing and packaging carbon for $N_c > 3$ where we take the digital logic in 7nm  and further split the logic block into smaller chiplets each implemented in 7nm. The analog (IOs) and memory chiplets are in 14nm and 10nm, respectively. Fig.~\ref{fig:cfp-nc-chiplets} shows the manufacturing and packaging CFP for different $N_c$. As $N_c$ increases, the chiplet manufacturing CFP decreases due to smaller chiplets and better yields, while the packaging CFP increases due to larger HI overheads. 



\noindent
%\textit{(5)} \underline{\it Packaging CFP for different architectures}
%To understand the differences in CFP overheads of the four different packaging architectures considered, we use the large digital logic component of GA102 as an example testcase. We split the 500mm$^2$ monolithic digital logic block into $N_c$ different chiplets and evaluate $C_\text{HI}$. Fig.~\ref{fig:package-cfp} shows the difference in CFP for these architectures separated by routing overheads and package-related overheads (whitespace and area).  For the four architectures, all the interconnects in the package substrate are modeled in a 65nm technology.  

%Silicon-bridge-based (EMIB-based) architectures have the least CFP for 2- and 4-chiplet-based architectures of the 500mm$^2$ monolith testcase. However, as $N_c$ increases, the number of silicon bridges also increases, and CFP increases. The RDL-based packages have the least overheads for the 6- and 8-chiplet architectures, but due to their architecture definition, they have lower communication bandwidth when compared to silicon bridges or interposers. Therefore, based on the bandwidth requirements of the testcase, such tradeoffs between performance and CFP can be considered using our analysis tool. The figure also shows that the passive interposer has lower routing overheads as the router is part of the chiplet and is in the same technology node of the chiplet. Therefore, in passive interposer technologies, due to the advanced node (7nm in this testcase) in which the router is implemented, the area overheads are smaller when compared to the 65nm router in the active interposer. The routing overheads of RDL, passive interposer, and silicon-bridge (EMIB) architectures are small and near-negligible when compared to the core chiplet areas.  

%\begin{figure}
%\centering
%\includegraphics[width=0.78\linewidth]{figs/package-cfp-overhead.png}
%\vspace{-5mm}
%\caption{Packaging CFP overheads for different $N_c$ values.}
%\vspace{-6mm}
%\label{fig:package-cfp}
%\end{figure}


\begin{comment}
\begin{table}[t]
\centering
\caption{Embodied CFP (grams of CO$_2$ emission) for chiplet-based and monolithic versions of industry testcases.}
\label{tbl:configurations}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccccc
}
\hline
Carbon    & EMR 2-chiplet & EMR 4-chiplet & GA102 & Apple A15 & Tiger Lake \\ \hline
$C_{\text{mfg},\text{chiplet1}}$ & 5.49E+04   & 2.06E+04   & 1.92E+03   & 1.28E+02   & 4.81E+02   \\
$C_{\text{mfg}, \text{chiplet2}}$ & 5.49E+04   & 2.06E+04   & 1.40E+03   & 4.17E+02   & 2.44E+02   \\
$C_{\text{mfg}, \text{chiplet3}}$ & --          & 2.06E+04   & 9.62E+03   & 1.53E+03   & 4.95E+02   \\
$C_{\text{mfg}, \text{chiplet4}}$ & --          & 2.06E+04   & 9.62E+03   & 1.53E+03   & --          \\ \hline
$C_\text{HI, RDL}$ & 7.49E+03   & 9.95E+03   & 2.78E+03   & 5.99E+02   & 2.40E+02   \\ 
 $C_\text{HI, EMIB}$ & 9.63E+02   &   2.22E+03 & 1.47E+03   & 7.30E+02   &  4.87E+02  \\
$C_\text{HI, passive}$ & 9.98E+03   & 1.33E+04   & 3.70E+03   & 7.93E+02   & 3.15E+02   \\
$C_\text{HI, active}$ & 1.00E+04   & 1.34E+04   &  3.76E+03  &  8.41E+02  & 3.49E+02   \\ \hline
$C_{\text{des}}$ & 1.19E+04	& 1.39E+04 &	4.70E+03 &	1.13E+03 &	2.63E+02
  \\ \hline \hline 

{\bf CFP$_{tot}$ (RDL)} &  1.29E+05	& 1.06E+05 &	3.00E+04 & 5.34E+03 &	1.72E+03
\\
{\bf CFP$_{tot}$ (EMIB)} & 1.23E+05 &	9.85E+04 &	2.87E+04 &	5.47E+03 &	1.97E+03
\\
{\bf CFP$_{tot}$ (passive)} & 1.32E+05 &	1.10E+05 &	3.10E+04 &	5.53E+03 &	1.80E+03
\\
{\bf CFP$_{tot}$ (active)} & 1.32E+05 &	1.10E+05 & 3.10E+04 &	5.58E+03 &	1.83E+03
\\ \hline  \hline 

{\bf Monolithic}  & {\bf 2.55E+05} &	{\bf 2.91E+05} &	{\bf 5.58E+04} &	{\bf5.60E+03} &	{\bf1.96E+03}
\\ \hline \hline 
\end{tabular}%
}
\vspace{-6mm}
\end{table}
\end{comment}


%\subsection{Summary for different testcases}
%In Table~\ref{tbl:configurations}, we compare the embodied (design, HI, and manufacturing) CFP  of a HI-based architecture against their monolithic SoC counterparts for different testcases, different packaging architectures, and a specific configuration of chiplets. The EMR 2-chiplet represents the architecture of the Intel Emerald Rapids (EMR) testcase, where both chiplets are in 7nm technology nodes. We create an EMR 4-chiplet testcase  where we further split the two chiplets in EMR into four based on the Intel Sapphire Rapids architecture~\cite{wiki-saphire-rapids}, all implemented in a 7nm technology. 
%The table also lists 4-chiplet versions of NVIDIA GPU GA102, and Apple A15 SoC, where the memory is implemented in 10nm, IOs/analog chiplets are implemented in 14nm, and the two digital logic chiplets in 7nm. The Tiger Lake testcase split into three chiplets for memory (10nm), analog (14nm), and digital logic (7nm).

%For the above-described testcases, the table lists $C_\text{mfg}, i$ for each chiplet, $C_\text{HI}$ for different packaging architectures, the $C_\text{des}$ assuming $N_\text{des} = 100$ and $N_p =200,000$, and the total CFP for each testcase compared against its monolithic counterpart.  We find that the total CFP of the HI-based testcases are all lower than their monolithic counterparts. For instance, the EMR 2-chiplet and 4-chiplet testcases with silicon bridge-based packages have 55\% and 70\% lower CFP when compared to their monolithic counterparts. We also observe that HI systems have a higher benefit with embodied CFP for large SoC testcases when compared to the smaller ones. For example, the GA102, and EMR testcases have large monolithic areas of approximately 500mm$^2$ and 1500mm$^2$, respectively, while the Apple A15 and Tiger Lake testcases have areas of over 100mm$^2$, and therefore the larger testcases, have a significantly higher improvement in CFP.

% We observe that HI-based systems have significantly lower CFP in larger monolithic SoC testcases (GA102, EMR) when compared to the smaller (Tiger Lake, A15) ones as large monolithic SoCs have lower yields that dominate any overheads in CFP due to HI-related reasons.  





